Analysis of GRB Closure Relationship in Multi-wavelengths

Gamma-ray bursts (GRBs) are intense pulses of high-energy emission associated with massive stars' death or compact objects' coalescence. Their multi-wavelength observations help verify the reliability of the standard fireball model. We analyze 14 GRBs observed contemporaneously in gamma-rays by the \textit{Fermi} Large Area Telescope (LAT), in X-rays by the \textit{Swift} Telescope, and in the optical bands by \textit{Swift} and many ground-based telescopes. We study the correlation between the spectral and temporal indices using closure relations according to the synchrotron forward-shock model in the stratified medium ($n \propto r^{-k}$) with $k$ ranging from 0 to 2.5. We find that the model without energy injection is preferred over the one with energy injection in all the investigated wavelengths. In gamma-rays, we only explored the $\nu > $ max\{$\nu_c,\nu_m$\} (SC/FC) cooling condition (where $\nu_c$ and $\nu_m$ are the cooling and characteristic frequencies, namely the frequencies at the spectral break). In the X-ray and optical bands, we explored all the cooling conditions, including $\nu_m < \nu < \nu_c$ (SC), $\nu_c < \nu < \nu_m$ (FC), and SC/FC, and found a clear preference for SC for X-rays and SC/FC for optical. Within these cooling conditions, X-rays exhibit the highest rate of occurrence for the density profile with $k = 0$, while the optical band has the highest occurrence for $k$ = 2.5 when considering no energy injection. Although we can pinpoint a definite environment for some GRBs, we find degeneracies in other GRBs.

==> old_tables.tex <==
\startdata
080916C & BPL & $1.609 \pm 0.213$ & $0.359 \pm 0.283$ &$0.860 \pm 0.536$ \\
090328A & BPL & $0.730 \pm  0.430$ & $1.058 \pm 0.141$ & $1.204 \pm 0.131$ \\ 
090510A & BPL & $2.316  \pm0.175$ &  $1.341 \pm  0.180$ & $1.052 \pm 0.063$ \\
090902B & BPL & $1.866 \pm  0.170$ & $1.237 \pm 0.231$ & $0.941 \pm 0.042$ \\
090926A & BPL & $1.765 \pm 0.168$ & $1.103 \pm 0.171$ & $1.138 \pm 0.054$ \\
100414A & BPL & $1.804 \pm 0.217$ &  $0.315 \pm 0.550$ & $0.801 \pm 0.118$ \\
110731A & BPL & $1.771 \pm 0.114$ & $0.389 \pm 1.071$ & $1.288 \pm 0.155$ \\
120711A & PL & - & $1.629 \pm 0.236$ & $1.058 \pm  0.167$ \\
130427A & BPL & $0.789 \pm 0.161$ & $1.423 \pm 0.104$ & $0.986 \pm 0.039$ \\
160509A & BPL & $0.879 \pm 0.266$ & $1.338 \pm 0.303$ & $1.382 \pm 0.119$ \\
160625B & PL & - & $2.236 \pm 0.284$ & $1.352 \pm 0.074$ \\
170405A & PL & - & $1.266 \pm 0.011$ & $1.794 \pm 0.349$ \\
171010A & BPL & $2.240 \pm 0.733$ & $0.969 \pm 0.294$ & $1.043 \pm 0.129$ \\
180720B & BPL & $1.458 \pm 0.187$ & $3.198 \pm 0.564$ & $1.230 \pm 0.097$ \\
220101A & PL & - & $1.104 \pm 0.529$ & $1.535 \pm 0.248$ \\
221009A & BPL & $1.580 \pm 0.460$ & $0.850 \pm 0.230$ & $0.790 \pm 0.050$ \\
